DRFLM: Distributionally Robust Federated Learning with Inter-client Noise via Local Mixup

Recently, federated learning has emerged as a promising approach for training a global model using data from multiple organizations without leaking their raw data. Nevertheless, directly applying federated learning to real-world tasks faces two challenges: (1) heterogeneity in the data among different organizations; and (2) data noises inside individual organizations. In this paper, we propose a general framework to solve the above two challenges simultaneously. Specifically, we propose using distributionally robust optimization to mitigate the negative effects caused by data heterogeneity paradigm to sample clients based on a learnable distribution at each iteration. Additionally, we observe that this optimization paradigm is easily affected by data noises inside local clients, which has a significant performance degradation in terms of global model prediction accuracy. To solve this problem, we propose to incorporate mixup techniques into the local training process of federated learning. We further provide comprehensive theoretical analysis including robustness analysis, convergence analysis, and generalization ability. Furthermore, we conduct empirical studies across different drug discovery tasks, such as ADMET property prediction and drug-target affinity prediction.

==> back.tex <==
\section{Theoretical Guarantees: }
The following theorems are informal results (which is in fact some existing results in other literature) about our Algorithm~\ref{algorithm:1}.

\begin{theorem}[Non-Convex Convergence Guarantee] It is guaranteed that after $T$-step iterations, \begin{align*}
    \min_{t = 1,\dots, T}\E[\lVert \nabla {f}\rVert_2 ] = O(T^{-1/4}).
\end{align*} 
\end{theorem}
\begin{remark}
In non-convex loss, we can only establish the vanishing rate of the gradient. This is in fact the direct application of Theorem~2 in \cite{dengDistributionallyRobustFederated2020}. 
\end{remark}
\begin{theorem}[Excess Risk] It is guaranteed that the minimizer after the mix-up distribution $\hat{w}$ of the loss $L_n$ satisfies \begin{equation}
    \E[L_n(\hat{w})]-\mathcal{L}(w^*) = O(\dfrac{1}{\sqrt{n}}).
\end{equation}
\end{theorem}


\section{Theorectical Model}
Our one layer GNN model is 
\begin{equation}
\hat{y}_{j}=\mathbf{a}_{j} \sigma\left(\mathbf{D}_{j}^{-1} \mathbf{A}_{j} \mathbf{H}_{j} \mathbf{W}\right) \mathbf{v}
\end{equation} 
while the underlying model is 
\begin{equation}
y_{j}=\mathbf{a}_{j} \sigma\left(\mathbf{D}_{j}^{-1} \mathbf{A}_{j} \mathbf{H}_{j} \mathbf{W}_{*}\right) \mathbf{v}_{*}+\epsilon_{j}
\end{equation}
where $\epsilon_j$ is independent sub-Gaussian noises, $\sigma$ is the activation function, $D_j\in \mathbb{R}^{n_j\times n_j}$ is the degree matrix of $j$-th graph, and $A_j\in \mathbb{R}^{n_j\times n_j}$ is the corresponding adjacency matrix, $W\in \mathbb{R}^{d\times d_{\text{out}}}$ is the local transition function which is shared among different nodes across different graphs.

For simplicity, we assume that the learning process for $W$ and $v$ is disjoint from that for $a_j$, or $a_j$ is ﬁxed and does not need training.

\begin{assumption}
$\sigma$ is a non-trivial increasing function, and is 1-Lipschitz continuous, i.e., $\left|\sigma\left(x_{1}\right)-\sigma\left(x_{2}\right)\right| \leq$ $\left|x_{1}-x_{2}\right|, \forall x_{1}, x_{2} \in \mathbb{R}$
\end{assumption}

\begin{assumption}
$\|\sigma(x)\|_{2} \leq L_{\sigma}\|x\|_{2}, \forall x \in \mathbb{R}^{n}$
\end{assumption}



abstract

Deep graph learning based drug discovery has demonstrated its potentiality to
accelerate traditional drug development pipeline. However, the training of deep graph models always requires large amounts of high-quality molecular data which is impractical in most of real-world scenarios. Federated learning emerges as a promising
way to train a model by utilizing data from multiple organizations without leaking
their raw data. However, directly applying federated learning to drug discovery tasks
faces two challenges: (1) data heterogeneity among different organizations (2) data noises inside local organizations. 

In this paper, we propose a general framework to solve the above two challenges
simultaneously. Specifically,  To mitigate the negative effect caused by data heterogeneity, we propose to employ distributionally robust optimization
paradigm to sample clients based on a learnable distribution at each iteration. 
Further, we observe that this optimization paradigm can be easily affected by data noises inside local clients thus has a significant performance degradation in terms of 
global model prediction accuracy. To solve this problem, we propose to incorporate mixup
techniques into the local training process of federated learning. We further provide comprehensive 
theoretical analysis including convergence speed, optimization efficiency and generalization ability. We also perform empirical studies across different drug discovery tasks including ADMET property prediction and DTI prediction.

Deep graph learning based on graph neural networks (GNNs) has achieved remarkable progresses in various drug discovery related tasks including molecular property prediction\cite{MolecularNet,MPNN}, protein-protein interaction (PPI) prediction \cite{PPI_prediction} and drug-target activity prediction \cite{} \bz{adding some refs}. Previous research in this direction has shown great potentiality to accelerate the drug discovery pipeline \cite{}\bz{add refs}. However, the training of GNNs always requires large amounts of high-quality molecular data and associated label information. This is impractical in most of real-world scenarios wherein data are distributed on different pharmaceutical companies and cannot be exchanged due to data regulations and business concerns (i.e., information silo issue) \cite{fl-qsar,xiongfeddrug}. 

To mitigate this information silo issue in deep learning, federated learning~(FL) emerges
as a promising way to enhance the model performance by utilizing data from multiple organizations without 
leaking their raw data. Specifically, there are some initial attempts to employ federated learning for drug discovery related
tasks \cite{fl-qsar,fedgnn,xiongfeddrug}. For example, Chen et al. \cite{fl-qsar} proposes FL-QSAR for cooperative quantitative structure-activity relationship (QSAR) analysis. He et al. \cite{fedgnn} proposes a federated GNN learning framework for various molecular property prediction tasks. However, most existing work  tries to directly apply conventional FL methods such as FedAvg \cite{fedavg} to real-world drug discovery tasks  without considering inherent properties of drug data \bz{adding refs}. 

In general, directly apply conventional FL methods to drug discovery faces two
critical challenges: (1) \emph{Inter-client data heterogeneity} (2) \emph{Intra-client data noise}.
Specifically, inter-client data heterogeneity refers to data from different clients always have various
distribution. This is also called Non-IID issue in the FL research community \cite{Scaffold,Fedprox}. For example, in the case of the drug-protein interaction prediction task, different pharmaceutical companies (labs) could  
have different high throughput  screening  environments when measuring the protein-ligand binding affinity, thus resulting in diverse assays in DTI data \bz{add refs}. 
% can have xxxx(assay and scaffold). 
Intra-client data noise refers to the noise generated in the process of data collection within each specific client.
A common noise source in drug discovery is the \emph{label noise} caused by measurement noise, or the situation where very low/high affinity values are often encoded as a boundary constant \bz{add refs}.  

There are a plenty of work aiming to solve the first issue \cite{mohri_agnostic_2019,reisizadeh_robust_2020,Fedprox,Scaffold,ditto,fed_non_iid_graph}. A typical research line is to employ adaptive training paradigm to improve the FL performance in the Non-iid setting (i.e., inter-client data heterogeneity).
For example, prior work \cite{reddi2021adaptive} proposes an adaptive optimizer for local model updating (e.g., Adam \cite{kingma2015adam} and AdaGrad \cite{duchi2011adaptive}) which allows to implicitly adjust local learning rate according to the loss function computed based on local data. However, most  work in this line needs to tune large amounts of  hyper-parameters of adaptive training paradigm to ensure model performance for different datasets, which is very challenging in real-world applications especially in the drug discovery tasks. A more general and essential way to overcome the client  heterogeneity is to incorporate distributionally robust optimization (DRO) \cite{kwon_principled_2020,zhai_doro_2021} \bz{needs more representational works} into conventional FL paradigm \cite{mohri_agnostic_2019,deng_distributionally_2021}.  
DRFA \cite{deng_distributionally_2021} is a recent work that proposes to optimize the agnostic (distributionally robust) empirical loss, which 
combines different local loss functions with learnable weights. This method theoretically ensures that the learned model can perform well over the worst-case local loss combination. Previous work in this line has shown its effectiveness in deep neural network on some small-scale benchmarks (e.g., Fashion MNIST). 

However, when we apply these methods
to real-world drug discovery tasks, we observe that these methods suffers from poor performance and training instability. Through extensive empirical studies, we identify that \emph{Intra-client data noise} inside the local client data is the main cause of the above issues ((adding some experiments figs)). Similar issues have also been discussed in the centralized setting \cite{zhai_doro_2021}. Several  work \cite{zhai_doro_2021} points out DRO is sensitive to outlier which further hinders model performance. In this paper, we focusing on mitigating the effects caused by intra-client data noise in the FL setting.

To solve the above two critical challenges in drug discovery, we present a general framework named \rfdd for building robust GNN models for a wide range of drug development tasks (e.g., molecular property prediction and drug-target interaction prediction) in the FL setting, i.e., joint modeling learning over
different organizations without leaking raw data. To overcome the inter-client data heterogeneity, we propose to employ DRO techniques to optimize the global model.
As discussed above, such a DRO method can be easily effected by intra-client data noise.
To mitigate negative effect caused by local noise, we propose to incorporate mixup \cite{zhang_mixup_2018} into local training process. We further provide comprehensive theoretical analysis including how introducing mix-up can  prevent local noise influence in DRFA while still maintain the cross-client robustness of DRFA and the convergerence guarantee of the proposed algorithm  \bz{xuxuan add some derivations} in Section \ref{sec: theory sec}. Following theoretical analysis, we conduct extensive empirical studies over a wide range of drug discovery tasks including molecular
property prediction and drug-protein interaction prediction. Results show the effectiveness in improving the out-of-distribution generalization ability and reducing the effects of local data noise.


(Under construction, illustrating different kinds of noises in drug AI datasets): 
There are several categories of noise from the area of AI-aided drug discovery, e.g, for CHEMBL \citep{mendez2019chembl}:  measurement noise, narrow measurement range,   low/high values are often only encoded as a boundary constant et al.   





Our contributions are summarized as follows:
\begin{itemize}
    \item consider two types of noises
    \item theoretical analysis
    \item results
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figs/intro_compare.pdf}
    \caption{Average and worst-case client RMSE of  FedAvg\cite{fedavg} and DRFA \cite{deng_distributionally_2021} on a molecular property prediction task. }
    \label{fig:my_label}
\end{figure}



==> related_works.tex <==
\nosection{Distributional Robust Learning in Federated Learning}
Recently, there are also several other works considering the data-heterogeneity across different clients. \cite{mohri_agnostic_2019} propose the concept of "agnostic federated learning", they shows that the empirical risk minimizer $\hat{f} $ of $\sum_{i=1}^m \alpha_i f_i(w)$  may have a  constant lower bound in the worst-case loss  \begin{equation}\label{worst-case loss} \max_{\lambda\in \Lambda} \sum_{i=1}^m \lambda_i f_i(w).\end{equation}  
Their work suggest to minimize  \eqref{worst-case loss} via alternatively update $w$ and $\lambda$, both the convergence guarantee for such algorithm and generalization bounds of performing ERM on \eqref{worst-case loss} has been established in their work. 
Later, \cite{deng_distributionally_2021} considered an algorithm minimizing \eqref{worst-case loss} in federated setting with less communication costs and establish the corresponding convergence guarantee in both convex and non-convex with strongly concave settings for their algorithm.
However, both works didn't deal with the data noise in local clients. 
There are fewer works consider the local noise in federated setting, \cite{reisizadeh_robust_2020} considered the robust federated learning with respect to local noise by taking local data augmentation. 
Their data augmentation method is to do the adversarial affine transformation, both the generalization guarantee and the optimization guarantee has been established in their paper.
However, while affine transformations are appealing for data with rotation-invariant properties, it  seems unreasonable to use such transformation family in our setting.  \\  
From the aspect of optimization guarantees, most of above works are based on the alternatively ascent-descent algorithms. The convergence of such algorithm for convex-concave minimax losses has been well established before. In practical the loss can be more complicated, \cite{deng_distributionally_2021}   considered the non-convex-concave loss under the PL condition, their analysis based on the technique developed in \cite{lin_gradient_2021}. The loss proposed in \cite{reisizadeh_robust_2020} is non-convex non-concave, and their proof in the convergence guarantee borrows ideas from the recent literatures \cite{nouiehed_solving_2019,yang_global_2020}.  

\textbf{Mix-up methods: } 
The mix-up method is proposed in \cite{zhang_mixup_2018} as an simple and efficient data-augmentation mechanism. 
There are a lot of sequential works demonstrate its improvement on robustness and generalization theoretically or empirically in many tasks\cite{zhang_how_2021,zhang_understanding_2017,carratino_mixup_2020,verma_interpolation_2020}. 
That also motivates a line of works for developing  a number of variants of Mixup, including the AdaMixUp\cite{guo_mixup_2018}, CutMix\cite{yun_cutmix_2019}, ManifoldMix\cite{verma_manifold_2019}, GraphMix\cite{verma_graphmix_2020,wang_mixup_2021}. 
Among them, \cite{verma_manifold_2019,verma_graphmix_2020,wang_mixup_2021} can be applied to graphical data, and the algorithm proposed in our work is an federated generalization of the approach in \cite{verma_manifold_2019}. 

\textbf{Distributional Robust Optimization: }
In stochastic optimization problem, we usually consider the minimizer of the problem $\inf _{h \in \mathcal{H}} R\left(\mathbb{P}_{\text{true}}, h\right)$ where $\mathbb{P}_{\text{true}}$ is the true distribution, $\mathcal{H}$ is a set of losses and $R(\mathbb{Q}, h):=\int h(\zeta) d \mathbb{Q}(\zeta)$.
While in real-world application, the computation is infeasible since the true distribution $\mathbb{P}_{\text{true}}$ is unknown or the integration is high-dimensional and thus computational expensive.
We instead observe a set of independent and identical distributed samples $Z=\{z_1,\cdots, z_n\}$ from the true distribution $\mathbb{P}_{\text{true}}$ in which we denote the empirical distribution of the samples as $\mathbb{P}_{\text{da ta}}$ and thus we solve the empirical risk minimization problem $\inf _{h \in \mathcal{H}} R\left(\mathbb{P}_{n}, h\right)=\inf _{h \in \mathcal{H}} \frac{1}{n} \sum_{i=1}^{n} h\left(z_{i}\right)$ where $\mathbb{P}_{n}:=n^{-1} \sum_{i=1}^{n} \delta_{z_{i}}$ is the empirical data distribution and $\delta_{z}$ is the Dirac delta distribution concentrating unit mass at $z$.
This replacement often yields poor risk estimation, and thus a solution to the empirical risk minimization can have a small training error but a large test error.
Wasserstein distributionally robust optimization (WDRO) is a popular option for preventing overfitting. The WDRO is formulated as $\inf _{h \in \mathcal{H}} \sup _{\mathbb{Q} \in \mathfrak{M}_{\alpha_{n}, p}\left(\mathbb{P}_{n}\right)} R(\mathbb{Q}, h)$ where $\mathfrak{M}_{\alpha_{n}, p}\left(\mathbb{P}_{n}\right)$ be a set of probability measures whose $p$-Wasserstein metric from $\mathbb{P}_{n}$ is less than $\alpha_{n}>0 .$ 
\cite{lee2017minimax} proves a minimizer of the WDRO problem has a vanishing excess worst-case risk bound when $\mathcal{H}$ is a set of Lipschitz continuous losses. More specifically, let $\hat{h}_{\alpha_{n}, p}^{\text {worst }}=\operatorname{argmin}_{h \in \mathcal{H}} R_{\alpha_{n}, p}^{\text {worst }}\left(\mathbb{P}_{n}, h\right)$ be the minimizer of the WDRO in empirical distribution and $R_{\alpha_{n}, p}^{\text {worst }}\left(\mathbb{P}_{\text {data }}, h\right)=\sup _{\mathbb{Q} \in \mathfrak{M}_{\alpha_{n}, p}\left(\mathbb{P}_{\text {data }}\right)} R(\mathbb{Q}, h)$ is the risk of the true underlying distribution. \cite{lee2017minimax} proves the risk consistency result $\mathcal{E}_{\alpha_{n}, p}^{\text {worst }}\left(\hat{h}_{\alpha_{n}, p}^{\text {worst }}\right)=O_{p}\left(n^{-1 / 2}\left(\mathfrak{C}(\mathcal{H}) \vee \alpha_{n}^{1-p}\right)\right)$ where $\mathcal{E}_{\alpha_{n}, p}^{\text {worst }}(g):=R_{\alpha_{n}, p}^{\text {worst }}\left(\mathbb{P}_{\text {data }}, g\right)-\inf _{h \in \mathcal{H}} R_{\alpha_{n}, p}^{\text {worst }}\left(\mathbb{P}_{\text {data }}, h\right)$.
While in general exactly solving WDRO is intractable since it involves the supremum operator over infinite many probability distributions, two streams of literature to handle it by using either a primal-dual pair of infinite-dimensional linear programs \cite{esfahani2018data} or first-order optimality conditions of the dual. In particular, \cite{gao2017wasserstein} shows that the local worst-case risk can be represented by a penalty-based methods, i.e., $R_{\alpha_{n}, p}^{\text {worst }}\left(\mathbb{P}_{n}, h\right)=\min _{\lambda \geq 0}\left\{\lambda \alpha_{n}^{p}+\frac{1}{n} \sum_{i=1}^{n} \sup _{z \in \mathcal{Z}}\left\{h(z)-\lambda\left\|z-z_{i}\right\|^{p}\right\}\right\}$. However, \cite{gao2017wasserstein} do not provide risk consistency result, which is not amendable by using \cite{lee2017minimax}'s proof trick since they have conflicting assumptions on $\mathcal{Z}$. In stead, \cite{kwon2020principled} propose the approximation $R\left(\mathbb{P}_{n}, h\right)+\alpha_{n}\left\|\nabla_{z} h\right\|_{\mathbb{P}_{n}, p^{*}}$ and prove its consistency, which is comparable to the results obtained in \cite{lee2017minimax}.
